Robust Sample-Based Output-Feedback Path Planning

We propose a novel approach for sampling-based and control-based motion planning that combines a representation of the environment obtained via a modified version of optimal Rapidly-exploring Random Trees (RRT*), with landmark-based output-feedback controllers obtained via Control Lyapunov Functions, Control Barrier Functions, and robust Linear Programming. Our solution inherits many benefits of RRT*-like algorithms, such as the ability to implicitly handle arbitrarily complex obstacles, and asymptotic optimality. Additionally, it extends planning beyond the discrete nominal paths, as feedback controllers can correct deviations from such paths, and are robust to discrepancies between the map used for planning and the real environment. We test our algorithms first in simulations and then in experiments, testing the robustness of the approach to practical conditions, such as deformations of the environment, mismatches in the dynamical model of the robot, and measurements acquired with a camera with a limited field of view.

==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=-1pt}


==> preamble/courseExam.tex <==
\usepgflibrary{shapes.arrows}

\input{preamble/courseFormatting}
\usepackage{probsoln}
\tikzset{ax/.style={very thick,-latex},pnt/.style={minimum size=5pt,fill=blue,circle,inner sep=0pt}}

%ref: https://tex.stackexchange.com/questions/201197/latex-using-the-matching-environment-in-the-exam-documentclass
\usepackage{multicol}

\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\fullwidth{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}
\newcommand{\vspacefivelines}{\vspacebox{6}}
\newcommand{\vspacesixlines}{\vspacebox{7}}
\newcommand{\vspacesevenlines}{\vspacebox{8}}

%% Create a Matching question format
\newcommand*\Matching[1]{
\ifprintanswers
    \textbf{#1}
\else
    \rule{2.7in}{0.5pt}
\fi
}
\newlength\matchlena
\newlength\matchlenb
\settowidth\matchlena{\rule{2.7in}{0pt}}
\newcommand\MatchQuestion[2]{%
    \setlength\matchlenb{\linewidth}
    \addtolength\matchlenb{-\matchlena}
    \parbox[t]{\matchlena}{\Matching{#1}}\enspace\parbox[t]{\matchlenb}{#2}}


==> preamble/courseFormatting.tex <==
%make underscore work without escaping in text mode
\usepackage{underscore}

%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue3}\sffamily}

%Perfect 1-inch margins
\usepackage[margin=1in]{geometry}
\usepackage[medium,compact]{titlesec}
\usepackage{longtable}
\titleformat*{\section}{\titlestyle \Large}
\titleformat*{\subsection}{\titlestyle \large \itshape}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}

%Displayed quotations (used to define an environment for function specification)
\usepackage{csquotes}


%Include code
\usepackage{listings}

%formatting for the description of a function's input/output arguments
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}

\newcommand{\dstar}{$\bigstar$}


==> preamble/courseProblemSet.tex <==
\input{preamble/courseFormatting}

%Facilities for markers file
% open file the beginning of the document
\AtBeginDocument{%
  \newwrite\markerstream
  \immediate\openout\markerstream=\jobname.mlg
}
% close the file at the end of the document
\AtEndDocument{%
  \immediate\closeout\markerstream
}
%definition similar to \typeout, but for markers
\makeatletter
\newcommand{\markerout}[1]{\begingroup \set@display@protect \immediate \write \markerstream {#1}\endgroup}
\makeatother

\usetikzlibrary{intersections}

\titleformat{\section}{\titlestyle\large\bfseries}{Problem \thesection:}{0.5ex}{}
%\titleformat{\subsection}{\normalfont\bfseries}{Problem \thesubsection:}{0.5ex}{}
\titleformat{\paragraph}[runin]{\titlestyle\normalsize\bfseries}{}{2pt}{}

%Macro for paragraph header for preparation steps to questions
%\newcommand{\preparation}{\smallskip\par\noindent\textbf{\titlestyle Preparation.~}}

\newcommand{\preparation}[1][]{%
\smallskip\par\noindent%
\textbf{\titlestyle Preparation\displayifnotempty{~(}{#1}{)}.~}}

%New custom counter for question
\newcounter{question}[section]

%Macro for writing points for the current question to the log file.
\newcommand{\pointmarker}{\typeout{Question points marker [\thesection.\thequestion] [\questionpoints]}}

\makeatletter
%Makes questions that:
%- are automatically numbered using the format <sectionNumber>.<questionNumber>
%- can be referred to using the usual \label-\ref mechanism
%- if the optional argument is not empty, this is displayed in parenthesis (typically, this will be a \points{n} or a \optional command). If the optional argument is empty, a single point is silently added to the point counter.
\newcommand{\question}[1][]{%
  \smallskip\par\noindent%
  \refstepcounter{question}\zerovar{\questionpoints}%
  \sbox\boxifnotempty{\textbf{\titlestyle #1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
  \textbf{\titlestyle Question \thesection.\thequestion\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
  \ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
  \def\@currentlabel{{\thesection.\thequestion}}\pointmarker%
  \markerout{Marker question [nolabel] [\thesection.\thequestion]}}%

%Commands that defines a new `labeled' question, which uses a separate counter but the same total point count. A new label with the same name must be defined separately
\newcommand{\newquestionlabel}[1]{%
  \newcounter{question#1}[section]%
  \expandafter\newcommand\csname question#1\endcsname[1][]{%
    \smallskip\par\noindent%
    \refstepcounter{question#1}\zerovar{\questionpoints}%
    \sbox\boxifnotempty{\textbf{\titlestyle ##1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
    \textbf{\titlestyle Question \csname #1\endcsname~\thesection.\csname thequestion#1\endcsname\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
    \ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
    \def\@currentlabel{{#1~\thesection.\csname thequestion#1\endcsname}}\pointmarker%
    \markerout{Marker question [#1] [\thesection.\csname thequestion#1\endcsname]}}%
}
\makeatother

\newquestionlabel{code}
\newquestionlabel{report}
\newquestionlabel{optional}
\newquestionlabel{provided}
\newquestionlabel{image}
\newquestionlabel{video}

\newcommand{\hintquestion}[1]{\paragraph{Hint
    for question \ref{#1}:~}}
\newcommand{\hint}{\paragraph{Hint:~}}

\newcommand{\answer}[1][]{\smallskip\leavevmode\\\noindent\textbf{Answer \thesection.\thequestion#1:~}}

\newcommand{\updated}[1]{{\color{red} #1}}

\newcolorlabel{labeloptional}{DodgerBlue3}
\newcommand{\optional}{\labeloptional{optional}}
\newcolorlabel{labelprovided}{Orange1}
\newcommand{\provided}{\labelprovided{provided}}
\newcolorlabel{labelvideo}{Coral2}
\newcommand{\video}{\labelvideo{video}}
\newcolorlabel{labelimage}{DarkOrchid2}
\newcommand{\image}{\labelimage{image}}
\newcolorlabel{labelcode}{SlateBlue2}
\newcommand{\code}{\labelcode{code}}
\newcolorlabel{labelscan}{Chocolate3}
\newcommand{\scan}{\labelcode{scan}}
\newcolorlabel{labelnew}{OliveDrab3}
\newcommand{\lbnew}{\labelnew{new}}
\newcolorlabel{labelreport}{OliveDrab3}
\newcommand{\report}{\labelreport{report}}
\newcolorlabel{labelgoal}{Black}
\newcommand{\goal}{\labelgoal{Goal}}

\tikzset{point/.style={inner sep=0pt,fill=black,circle,minimum size=4pt}}

%macros for keeping track of points (total, and for current question)
\zerovar{\totalpoints}
\zerovar{\bonuspoints}
\zerovar{\questionpoints}
\newcommand{\increasepoints}[1]{\addtovar{\totalpoints}{#1}\addtovar{\questionpoints}{#1}}
\newcommand{\points}[1]{#1 point\ifthenelse{\equal{#1}{1}}{}{s}\increasepoints{#1}}
\makeatletter
\newcommand{\totalpointswithbonus}[1]{\pgfmathparse{\storeddef{totalpoints}+#1}\pgfmathresult\typeout{Total points marker [\pgfmathresult]}}
\makeatother

\newstoreddef{totalpoints} %remember total number of points in aux file

% answer boxes
\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\par\bigskip{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}
\newcommand{\vspacefivelines}{\vspacebox{6}}
\newcommand{\vspacesixlines}{\vspacebox{7}}

% text fields
\newcommand{\textrowfield}[1]{\par\noindent#1: \enspace\hrulefill}

% formatting for the description of a function's input/output arguments
\usepackage[framemethod=tikz]{mdframed}
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
\mdfdefinestyle{classspecification}{%
linecolor=DarkOliveGreen3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
%Note: I was not able to avoid duplication of options.

\newenvironment{functionspecification}{\markerout{Marker function [start]}\begin{mdframed}[style=functionspecification]}
{\markerout{Marker function [end]}\end{mdframed}}%
\newenvironment{classspecification}{\markerout{Marker class [start]}\begin{mdframed}[style=classspecification]}
{\markerout{Marker class [end]}\end{mdframed}}%
%\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\newenvironment{cdescription}{\fdescription}{\endfdescription}
\NewEnviron{frequirements}{\par\noindent{\titlestyle Requirements}: \BODY\markerout{Marker text [requirements] [start]^^J\BODY^^JMarker text [requirements] [end]}\par}
\newcommand{\cname}[1]{\noindent{\titlestyle Class name}: \var{#1}\par}
\newenvironment{finputs}{\markerout{Marker argument_group [start] [inputs]}\noindent{\titlestyle Input arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foptional}{\markerout{Marker argument_group [start] [optional]}\noindent{\titlestyle Optional arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foutputs}[1][Output]{\markerout{Marker argument_group [start] [outputs]}\noindent{\titlestyle #1 arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newcommand{\freturns}[2][]{\noindent{\titlestyle Returns}: \var{#2}\displayifnotempty{ (type }{\var{#1}}{)}}
\newcommand{\argument}[4][]{\markerout{Marker argument [start]}\markerout{Marker argument [name] [#2]}\var{#2} %
  \ifnotempty{#1#3}{(\ifnotempty{#3}{\markerout{Marker argument [dimensions] [#3] [#4]}dim. \vardim{#3}{#4}}%
  \ifnotempty{#1}{, \markerout{Marker argument [type] [#1]}type \var{#1}{}})}\markerout{Marker argument [end]}}
\newcommand{\argumentscalar}[2][]{\argument[#1]{#2}{}{}}
\newcommand{\fheader}[3][]{\noindent{\titlestyle Header}: \function[#1]{#2}{#3}\par}
\newcommand{\fname}[2][Function]{\noindent{\titlestyle #1 name}: \var{#2}\par}
\newcommand{\ffilename}[1]{\noindent{\titlestyle File name}: \file{#1}\par}
\newcommand{\functionheader}[3][]{\markerout{Marker function_header [#1] [#2] [#3]}\function[#1]{#2}{#3}\par}

% Commands to indicate functions and files that are provided but not fully specified
\newcommand{\mfunctionprovided}[3][]{\markerout{Marker file_provided [#2.m]}\function[#1]{#2}{#3}}
\newcommand{\fileprovided}[1]{\markerout{Marker file_provided [#1]}\file{#1}}
\newcommand{\fileincluded}[1]{\markerout{Marker file_provided [#1]}}
%note: fileprovided and fileincluded differ on whether the file name is inserted in the TeX output (in both cases, it is inserted in the marker log)

%ROS node specification
\newenvironment{nodespecification}{\begin{mdframed}[style=functionspecification]%
\newcommand{\filename}[1]{\par{\titlestyle File name:} \file{##1}}
\renewenvironment{description}{\par\noindent{\titlestyle Description:}}{\par}%
\newenvironment{subscribers}{\par\noindent{\titlestyle Subscribes to topics:}}{}%
\newenvironment{publishers}{\par\noindent{\titlestyle Publishes to topics:}}{}%
%
}{\end{mdframed}}

\newcommand{\rostopic}[2]{\var{#1} (type \var{#2})}

% Macros for questions where student need to draw on axes
\newcommand{\drawingaxes}[1][]{\draw[gray] (-5,-5) grid (5,5);
  \draw[very thick, -latex] (-5.7,0) -- (5.7,0) coordinate (a1);
  \draw[very thick, -latex] (0,-5.7) -- (0,5.7) coordinate (a2); #1}

\newcommand{\shifteddrawingaxes}[1][]{
  \begin{scope}[xshift=18cm]
    \drawingaxes[#1]
  \end{scope}
}

\newcommand{\drawexercise}[2][]{\begin{center}
\begin{tikzpicture}[scale=0.6]
  \node[text width=7cm,anchor=west]{#2};
  \shifteddrawingaxes[{\node at ($(a1)-(0,1.2em)$) {$x_1$}; \node at ($(a2)+(1.2em,0)$) {$x_2$}; #1}]
\end{tikzpicture}
\end{center}
}


==> preamble/courseProblemSetSectionsLettered.tex <==
%Change format of numbering for questions to letters instead of numbering
\renewcommand{\thequestion}{\alph{question}}


==> preamble/courseSyllabus.tex <==
\input{preamble/courseFormatting}
\usepackage{etoolbox}

\newlength{\topicwidth}
\newlength{\topicdatewidth}
\setlength{\topicdatewidth}{19mm}
\newlength{\duewidth}
\setlength{\duewidth}{23mm}

% Create a topictable environment from the longtable environment
\newenvironment{topictable}[1][2cm]%
{\newcommand{\picswidth}{#1}\setlength{\topicwidth}{\textwidth-\picswidth-\topicdatewidth-\duewidth-12.5mm}%
  \setcounter{topic}{1}\begin{longtable}{p{\picswidth}p{\topicwidth}p{\topicdatewidth}p{\duewidth}}}%
  {\end{longtable}}

% Prepare counter and relative macros for handling array of class dates
\newcount\i
\pgfmathsetcount{\i}{0}
\def\classdate{\pgfprint{\classdatearray[\i]}\global\advance\i 1\relax}

% Counters for topic and subtopic
\newcounter{topic}
\newcounter{subtopic}

% Toggle for controlling pod switching
\newtoggle{pod}
\toggletrue{pod}
\newcommand{\podtoggle}{\iftoggle{pod}{\pods{A,B}\global\togglefalse{pod}}{\pods{C,D}\global\toggletrue{pod}}}

% Labels
\newcolorlabel{labelhw}{Orange1}
\newcommand{\hwrel}[1]{\par\labelhw{HW #1 Rel}~}
\newcommand{\hwdue}[1]{\labelhw{HW #1}}
\newcolorlabel{paperdue}{Tomato1}
\newcolorlabel{examdue}{Tomato1}
\newcolorlabel{labelMH}{DodgerBlue3}
\newcommand{\mhday}{\labelMH{M-H}~}
\newcolorlabel{labelqz}{Sienna3}
\newcommand{\qzdue}[1]{\labelqz{QZ #1}~}
\newcommand{\activity}{\labelqz{Activity}~}
\newcommand{\readinggroup}{\labelqz{Reading group}~}
\newcolorlabel{labelpod}{DarkOliveGreen3}
\newcommand{\pods}[1]{\labelpod{Pods #1}~}
\newcommenter{instructor}{DarkOliveGreen3}



% Topichead
\def\topichead#1#2#3{\rowcolor{SlateGray1}{\setcounter{subtopic}{1}\rule{0pt}{16pt}\titlestyle Topic \arabic{topic}\addtocounter{topic}{1}} & \multicolumn{3}{l}{{\titlestyle #1:} #2 \rule[-8pt]{0pt}{12pt}}\\\tikz[overlay]{\node[anchor=north west,inner sep=0pt]{\includegraphics[width=\picswidth,keepaspectratio]{figures/#3}};}}
\def\firstsubtopic#1{ & \makecell[{{p{\topicwidth}}}]{\rule{0pt}{14pt}#1}\addtocounter{subtopic}{1}}
\makeatletter
\def\subtopic{\@ifstar\@subtopicstar\@subtopic}
\def\@subtopic#1{\\ \cmidrule{2-4} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
\def\@subtopicstar#1{\\ \cmidrule{2-2} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
\makeatother
\def\activitytopic#1{\\ \cmidrule{2-4} & \multicolumn{3}{l}{\parbox{\topicwidth+\topicdatewidth+\duewidth}{\activity #1}}}
% \def\topicdate#1{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\makeatletter
\def\topicdate{\@ifstar\@topicdatestar\@topicdate}
\newcommand{\@topicdate}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\newcommand{\@topicdatestar}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1 \podtoggle}}
\makeatother
\def\due#1{& \makecell[{{p{\duewidth}}}]{#1}}
\def\endtopic{\\}
% TODO: Add automatic test to check if a subtopic is the first subtopic, and adjust the formatting accordingly.
% The subtopic counter is already there, but due to conflicts with the tabular environment, I was not able to include the test inside the \subtopic macro.
% \def\tpctest{\noalign{\ifnum\value{subtopic}=1{}\else{\hrule}\fi}}


==> preamble/generateGraphLocalization <==
#!/usr/bin/env python
# Note: in the list of node and edge quantities: first element is the name to use in the command name,
# the second is the one to use in the definition

import os
f=open('graphLocalization.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Notation for nodes\n')
nodeIndexList=['i','j']
nodeStateDoubleList=[['R','R'],['T','T']]
for index in nodeIndexList:
    for state in nodeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
        f.write('\\newcommand{\\d'+state[0]+index+'}{\\dot{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dd'+state[0]+index+'}{\\ddot{'+state[1]+'}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

edgeIndexList=['ij','ji']
edgeStateDoubleList=[['R','R'],['T','T'],['beta','\\beta'],['c','c'],['d','d'],['q','q'],['l','\\lambda'],['varphi','\\varphi'],['g','g']]

f.write('% Notation for edges\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Notation for edges, measured quantities\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\t'+state[0]+index+'}{\\tilde{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dt'+state[0]+index+'}{\\dot{\\tilde{'+state[1]+'}}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Node state differences\n')
f.write('\\newcommand{\\xjmi}{x_j-x_i}\n')
f.write('\\newcommand{\\vjmi}{v_j-v_i}\n')
f.write('\\newcommand{\\nxjmi}{\\norm{\\xjmi}}\n')
f.write('\n')

f.write('% Notation for desired quantities\n')
quantityTripleList=[['x','x','i'],['x','x','j'],['beta','\\beta','ij'],['d','d','ij']]
for quantity in quantityTripleList:
    f.write('\\newcommand{\\'+quantity[0]+'g'+quantity[2]+'}{'+quantity[1]+'_{g,'+quantity[2]+'}}\n')

f.close()






        


==> preamble/generateNotation <==
#!/usr/bin/env python
import string
import os
f=open('notation.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Shortand notation for vectors and their derivatives\n')
for c in string.ascii_lowercase+string.ascii_uppercase:
    f.write('\\providecommand{\\v'+c+'}{\\vct{'+c+'}}\n')
    f.write('\\providecommand{\\dv'+c+'}{\\dot{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\tv'+c+'}{\\tilde{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\dtv'+c+'}{\\dot{\\tilde{\\vct{'+c+'}}}}\n')
f.write('\n')
for c in [['beta','\\beta'],['sigma','\\sigma']]:
    f.write('\\providecommand{\\v'+c[0]+'}{\\boldsymbol{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dv'+c[0]+'}{\\dot{\\boldsymbol{'+c[1]+'}}}\n')
f.write('\n')
for c in ['e']:
    f.write('\\providecommand{\\t'+c+'}{\\tilde{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for derivatives and bold of symbols\n')
for c in [['gamma','\\gamma'],['Delta','\Delta'],['pi','\pi']]:
    f.write('\\providecommand{\\d'+c[0]+'}{\\dot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dd'+c[0]+'}{\\ddot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\v'+c[0]+'}{\\bm{'+c[1]+'}}\n')
f.write('\n')


f.write('% Shortand notation for matrices\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\m'+c+'}{\\vct{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for calligraphic upper case letters\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\c'+c+'}{\\mathcal{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for some tilded symbols and their derivatives\n')
symbolDoubleList=[['x','x'],['y','y'],['varphi','\\varphi']]
for symbol in symbolDoubleList:
    f.write('\\providecommand{\\t'+symbol[0]+'}{\\tilde{'+symbol[1]+'}}\n')
    f.write('\\providecommand{\\dt'+symbol[0]+'}{\\dot{\\tilde{'+symbol[1]+'}}}\n')
f.write('\n')

f.close()


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}
\usepackage{cprotect}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[2][.]{\section{$\mathrm{#2}$}%
\tikzsetnextfilename{#2}%
  \begin{tikzpicture}[scale=0.7]%
    \input{#1/sketch/#2}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[2][.]{\section{$\mathrm{#2}$}%
\tikzsetnextfilename{#2}%
\input{#1/tikz/#2}%
\endpgfgraphicnamed%
}


==> preamble/math.tex <==
% AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
\usepackage[cmex10]{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
\usepackage{amsthm}%
}{}
\makeatother
% Generic symbols (e.g., \degree)
\usepackage{gensymb}
% Prescripts, squashed summations, and others
\usepackage{mathtools}
% Bold greek letters
\usepackage{bm}

%Common math statements environments
\makeatletter
\@ifundefined{theorem}{
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
}{}
  %SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{
  \newtheorem{definition}{Definition}
}
% \@ifundefined{remark}{
%   \newtheorem{remark}{Remark}
% }
\makeatother
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/posterCommon.tex <==
\input{preamble/posterGraphics}
\input{preamble/posterFormatting}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/posterFormatting.tex <==
%fonts
\usepackage[scaled=0.90]{helvet}
\usepackage{courier}

%sectioning
\pagestyle{empty}
\setcounter{secnumdepth}{0}

%headings
\def\Head#1{\noindent\hbox to \hsize{\hfil{\veryHuge\color{DarkBlue} #1}}\bigskip}
\def\LHead#1{\noindent{\LARGE\color{Blue} #1}\vspace{-.5cm}}
\def\Subhead#1{\noindent{\Large\color{DarkBlue} #1}\vspace{-.5cm}}
\def\Subsubhead#1{{\color{Blue} #1}}
\def\Title#1{\noindent{\Huge #1}}

%text boxes and grid
%Note: use options showboxes if you want to see the boxes
\usepackage[absolute]{textpos}
\TPGrid[30mm,30mm]{10}{20}  % 3 - 1 - 7 - 1 - 3 Columns

% Mess with these as you like
\parindent=0pt
%\parindent=1cm
\parskip=0.5\baselineskip


==> preamble/posterGraphics.tex <==
\usepackage{tikz}
\usepackage{xcolor}

%colors
\definecolor{Blue}{rgb}{0.05,0.2,0.5}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{LightBlue}{rgb}{.2431,.5451,.8588}
\definecolor{Red}{rgb}{1.0,0,0}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}

%for callouts
\usetikzlibrary{calc,chains,positioning,shapes.callouts}

%bullet points
\renewcommand{\labelitemi}{\color{LightBlue}{$\bullet$}}

%highlighting
\newcommand{\alert}[1]{{\color{LightBlue} #1}}

%rounded boxes
\newenvironment{roundboxes}[1][]
{\begin{tikzpicture}[start chain,node distance=2cm,
 every node/.style={on chain, text=black,fill=LightBlue!20, rounded corners=0.6cm},#1]
}
{\end{tikzpicture}
}

%Define anchors for callouts
\newcommand{\anchor}[1]{\tikz[remember picture] \coordinate (#1);}

%Insert callouts. Syntax:
%\callout[optionalStyle]{pointer}{positionRelativeToThePointer}{text}
\newcommand{\callout}[4][]{\begin{tikzpicture}[remember picture, overlay]
 \node[rectangle callout, fill=gray!50, #1, callout absolute pointer={#2}] at ($ #2 + #3 $) {#4};
\end{tikzpicture}
}

%Rounded box to highlight plus define anchor
\newcommand{\enboxref}[3][]{
  \tikz[baseline,remember picture]{
    \node[fill=gray!20,anchor=base,rounded corners=0.6cm,#1] (#2) {#3};
  }
}

%Boxes to define sections
\newlength{\sectionboxpadding}
\setlength{\sectionboxpadding}{5mm}

\newcommand{\sectionboxcolor}{LightBlue}

\newcommand{\sectionboxstart}[1]{\makebox[0cm][l]{\anchor{#1 a}}}
\newcommand{\sectionboxend}[1]{\makebox[0cm][l]{\anchor{#1 b}} \vspace{-3em}\\}
\newcommand{\sectionboxdraw}[2][]{\begin{tikzpicture}[remember picture, overlay,#1]
 \draw[rounded corners, line width=5pt, draw=\sectionboxcolor] ($(#2 a)+(0,0.6em)+(-\sectionboxpadding,\sectionboxpadding)+(0,0.4em)$) rectangle ($(#2 b)+(\textwidth,1em)+(\sectionboxpadding,-\sectionboxpadding)+(0,0.4em)$);
\end{tikzpicture}
}

\newcommand{\generalboxdraw}{
\begin{tikzpicture}[remember picture, overlay, LightBlue]
\draw[line width=5pt] ($(current page.north west) + (2,-13.5)$) rectangle ($(current page.south east) + (-2,3)$);
\end{tikzpicture}
}


==> preamble/preambleHelp.tex <==
\section*{Markup and commenting commands}
Use the command \var{\textbackslash newcommenter\{cname\}\{color\}} to enable the following commands (substitute \var{cname} with your pseudonim of choice, e.g., \var{rtron}, and \var{color} with a color name supported by the \var{xcolor} package):
\begin{itemize}
\item \var{\textbackslash cname\{comment\}}: typeset a colored comment labeled with the pseudonim.
\item \var{\textbackslash atcname}: use this to refer to another commenter.
\item \var{\textbackslash cnamehl\{comment\}\{text\}}: use this to highligth a portion of the text and comment on it.
\end{itemize}
Examples after using \var{\textbackslash newcommenter\{rtron\}\{Green3\}}:
\begin{itemize}
\item \var{\textbackslash rtron\{Ignore this comment\}} produces \rtron{Ignore this comment}.
\item \var{\textbackslash atrtron} produces \atrtron.
\item \var{\textbackslash rtronhl\{Sentence is obvious\}\{The sky is blue\}} produces \rtronhl{Sentence is obvious}{The sky is blue}
\end{itemize}

Use the command \var{\textbackslash sout} to strike out text.

Use \var{\tikztestgrid{4}{3}} to draw, inside a \var{tikzpicture}, a test grid 4 units wide, 3 units tall, and centered at (0,0).

==> preamble/proposals.tex <==

\input{preamble/compactLists}
\input{preamble/proposalsPagination}
\input{preamble/proposalsFormatting}
\input{preamble/splitting}

\newcommand{\testgrid}{\tikz[remember picture, overlay]{%
  \coordinate (tl) at  ($(current page.north west)+(1in,-1in)$);%
  \coordinate (br) at  ($(current page.south east)+(-1in,1in)$);%
  \draw[red] (tl) rectangle (br);%
  \draw[red] (tl) grid[xstep=2\textwidth,ystep=1in] (br);}}




==> preamble/proposalsAggressive.tex <==
\linespread{0.93}


==> preamble/proposalsEnableHelvetica.tex <==
%These commands set Helvetica as the default font
\usepackage[scaled]{helvet}
\renewcommand\familydefault{\sfdefault} 
\usepackage[T1]{fontenc}


==> preamble/proposalsFormatting.tex <==

\paragraphswithstop 

% Reduce line skip before \paragraph
\titlespacing{\paragraph}{%
  0pt}{%              left margin
  0\baselineskip}{%   space before (vertical)
  0.5em}%             space after (horizontal)


% Change name of section for references
\renewcommand{\refname}{References Cited}

%Redefine \maketitle command
\makeatletter
\renewcommand{\maketitle}{\begin{center}\Large\textbf\@title
  \end{center}
  % Add author only if not empty (in the sense of producing output)
\setbox0=\hbox{\@author\unskip}\ifdim\wd0=0pt
\else
\begin{center}
  \@author
\end{center}
\fi%
}
\makeatother

%theorem-like environment for stating thrusts
%we define a second counter that is updated in synch with the default
%one, but is presented in Alphabetic form
\newtheorem{innerthrust}{Thrust}
\newcounter{thrustnumber}
\newenvironment{thrust}[1][\Alph{thrustnumber}]
  {\stepcounter{thrustnumber}\renewcommand\theinnerthrust{#1}\innerthrust}
  {\endinnerthrust}


%macros for paragraphs in thrust description
\newcommand{\thrustmerits}{\paragraph{Intellectual merits of
    this thrust}}
\WithSuffix\newcommand\thrustmerits*[1][\Alph{thrustnumber}]{\paragraph{Intellectual merits of thrust~#1}}

\newcommand{\thruststateoftheart}{\paragraph{State of
    the art and open problems}}
\WithSuffix\newcommand\thruststateoftheart*[1][\Alph{thrustnumber}]{\paragraph{Relation of thrust~#1 with the state of the art}}

\newcommand{\thrustbackground}[1]{\paragraph{Background on #1}}

\newcommand{\thrustgoal}{\paragraph{Goal of this thrust}}

\newcommand{\proposalcontribution}[1]{\paragraph{Proposed innovation: #1}}

\newcommand{\collaborationletter}{\emph{Letter of collaboration}}

\setlist[description]{%
  font={\itshape}, % set the label font
}

\newenvironment{wrapremark}[2][]
{  \setlength{\intextsep}{0em}
  \wrapfigure{#2}{0.4\textwidth}\vspace{-0.5em}\mdframed\vspace{-3mm}\remark[#1]}
{\endremark\endmdframed\endwrapfigure}



==> preamble/proposalsNIH.tex <==
\input{preamble/proposalsEnableHelvetica}
\geometry{margin=0.5in}

==> preamble/proposalsPagination.tex <==
\usepackage{url}
\usepackage{times}

\usepackage[compact]{titlesec}

% Perfect 1 inch margins
\usepackage[letterpaper,margin=1in]{geometry}

%Make font for captions smaller (saves space and visually separates them from the main text)
\usepackage[font={footnotesize,sf}]{caption}

% Nice gantt charts
\usepackage{pgfgantt}



==> preamble/proposalsTaskSections.tex <==
%The following reformat the sections so that their labels read "Task x.y" instead of "x.y".
%Use the starred version of the command if you do not want this for
%some of the sections
\titleformat{\section}{\normalfont\large\bfseries}{Task \thesection:}{0.5ex}{}
\titleformat{\subsection}{\normalfont\bfseries}{Task \thesubsection:}{0.5ex}{}


==> preamble/proposalsTitles.tex <==
%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue4}\sffamily}

%Format titles
\titleformat*{\section}{\titlestyle \bfseries \Large}
\titleformat*{\subsection}{\titlestyle \bfseries \large}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}
\renewcommand{\paragraph}[1]{\par\noindent{\titlestyle\small\bfseries #1.~}}

% Format mdframed boxes
\mdfsetup{%
  middlelinecolor=DodgerBlue4,
  middlelinewidth=1pt,
  %backgroundcolor=red!10,
  roundcorner=3pt}

==> preamble/pysplitmaster <==
#!/usr/bin/python

""" Script that splits the file master.pdf produced by the NSF Proposal template into the individual parts required for submissions """

import re
import subprocess
from optparse import OptionParser

def main(options):
    baseFileName=options.filename

    #Open log file
    fileName=baseFileName+'.log'
    logFile = open(fileName,'r')

    if options.verbose:
        print 'fileName: ', fileName

    #Regexp for matching split markers
    reProg=re.compile('Split marker \[([\w\-]*)\] \[(start|end)\] \[(\d*)\]')

    #Check the log file line by line and add matches to list
    matchList=[]
    for (lineNb,line) in enumerate(logFile):
    	m=reProg.findall(line)
        if m:
       	   matchList+=m
           if options.verbose:
               print 'Match found on line', lineNb+1, ':', m

    if options.verbose:
        print 'matchList:'
        print matchList

    #Transform the match list into a double dictionary
    matchDict={}
    for m in matchList:
        if m[0] not in matchDict:
	    matchDict[m[0]]={}
	pageNumber=int(m[2])
	if m[1]=='end':
        #Split marker gives +1 page for end. Fix that
	    pageNumber-=1
	matchDict[m[0]][m[1]]=pageNumber

    if not checkMatchDict(matchDict):
        return -1

    pdfFileName=baseFileName+'.pdf'

    for sectionName,v in matchDict.items():
        #Split a section in its own file
        cmd=['pdftk', pdfFileName, 'cat', str(v['start'])+'-'+str(v['end']), 'output', sectionName+'.pdf']
        print cmd
        subprocess.check_call(cmd)

        #Strip all annotations
        cmd=['pdfStripAnnotations', sectionName+'.pdf']
        print cmd
        subprocess.check_call(cmd)

def checkMatchDict(matchDict):
    ''' Checks consistency of starts/ends for match dictionary '''
    for k,v in matchDict.items():
        #check presence of start and end
        if 'start' not in v:
            print 'Missing start for section '+k
            return False
        if 'end' not in v:
            print 'Missing end for section '+k
            return False
        if v['end']<v['start']:
            print 'Start/end page numbers for section '+k+' not consistent'
            return False
        return True

if __name__ == "__main__":
    parser = OptionParser()
    parser.add_option("-f", "--master-file", dest="filename",
        help="base name of the master file to split without extension",
        default="master")
    parser.add_option("-v", "--verbose",
        action="store_true", dest="verbose", default=False,
        help="print intermediate details")
    (options, args) = parser.parse_args()
    main(options)


==> preamble/reviewDraft.tex <==
\usepackage{background}
\backgroundsetup{contents={%
    \begin{tikzpicture}[overlay,font=\sffamily]
      % \newcommand{\scaletop}{-.68in}
      % \newcommand{\scalepitch}{1.15em}
      % \newcommand{\scaleoffset}{.5in}
      % \foreach \x in {1,...,60}{
      %   \node at ($(current page.north west)+(\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+\x)}\pgfmathresult};
      %   \node at ($(current page.north east)+(-\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+100+\x)}\pgfmathresult};
      % }
      \node at ($(current page.south)+(0,.5in)$) {*** For Review Only ***};
    \end{tikzpicture}
  },color=blue,scale=1,angle=0}
\let\bframe\relax %remove command from robotics.tex conflicting with lineno
\usepackage[displaymath, mathlines,switch]{lineno}
\linenumbers
\author{\textcolor{blue}{\sffamily Author Names Omitted for Anonymous Review}}
\renewcommand{\author}[1]{}


==> preamble/roboticsHelp.tex <==
This file introduces commands for drawing axes and cameras.

\begin{itemize}
\item \var{ax[label][opts]\{refid\}\{x\}\{y\}\{rot\}} Draws a pair of 2-D axes. \var{refid} can be the used to put labels and third axes.
\item \var{axup[label_rotation]\{refid\}\{label\}\{rot\}}
\item \var{axlabels\{refid\}\{label1\}\{label2\}}
\item \var{camera[label]\{refid\}\{x\}\{y\}\{rot\}}
\item \var{gpoint\{coordinates\}\{label\}\{rot\}}
\end{itemize}


==> preamble/splitting.tex <==
%Macro to include file while writing to log file the splitting markers
\newenvironment{markforsplit}[1]{%
  \def\splitmarkername{#1}
  \typeout{Split marker [#1] [start] [\theCurrentPage]}  \setcounter{page}{1}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
}{%
  \clearpage%
  \typeout{Split marker [\splitmarkername] [end] [\theCurrentPage]}%
}
\newcommand{\includeforsplit}[1]{%
\begin{markforsplit}{#1}%
\include{#1}%
\end{markforsplit}%
}

